RoboPol: AGN polarimetric monitoring data

We present uniformly reprocessed and re-calibrated data from the RoboPol programme of optopolarimetric monitoring of active galactic nuclei (AGN), covering observations between 2013, when the instrument was commissioned, and 2017. In total, the dataset presented in this paper includes 5068 observations of 222 AGN with Dec > -25 deg. We describe the current version of the RoboPol pipeline that was used to process and calibrate the entire dataset, and we make the data publicly available for use by the astronomical community. Average quantities summarising optopolarimetric behaviour (average degree of polarization, polarization variability index) are also provided for each source we have observed and for the time interval we have followed it.

==> table_sample_full.tex <==
 RBPLJ0006-0623 &      PKS 0003-066 &  00:06:13.9 &  $-$06:23:35.3 &                     0.34668 &  \cite{2009MNRAS.399..683J} &      5 &    v &   15 &  2 &   8 &  21.20 &  0.45 &  0.13 & -14.0 \\
 RBPLJ0017+8135 &        S5 0014+81 &  00:17:08.5 &  $+$81:35:08.1 &                       3.366 &  \cite{1994ApJ...436..678O} &    2,4 &    v &   30 &  3 &   7 &   0.80 &  0.62 &  0.65 &     - \\
 RBPLJ0035+5950 &      1ES 0033+595 &  00:35:52.7 &  $+$59:50:04.2 &                       0.086 &  \cite{1999AnA...352...85F} &      5 &    6 &    5 &  1 &   8 &      - &     - &     - &     - \\
 RBPLJ0045+2127 &                 - &  00:45:19.3 &  $+$21:27:40.0 &                           - &                           - &      3 &    v &   64 &  4 &   3 &   4.83 &  0.59 &  0.84 &     - \\
 RBPLJ0102+5824 &      TXS 0059+581 &  01:02:45.8 &  $+$58:24:11.1 &                       0.644 &  \cite{2005ApJ...626...95S} &      5 &    v &   18 &  3 &   9 &  13.45 &  0.32 &  0.53 &     - \\
 RBPLJ0114+1325 &                 - &  01:14:52.8 &  $+$13:25:37.5 &    0.583\textsuperscript{*} &  \cite{2014ApJ...784..151S} &      3 &    v &   59 &  4 &   4 &   7.04 &  0.48 &  0.74 &     - \\
 RBPLJ0136+3905 &       B3 0133+388 &  01:36:32.5 &  $+$39:05:59.6 &                       0.750 &  \cite{2015AnA...575A..21N} &      6 &    v &    7 &  2 &  27 &      - &     - &     - &     - \\
 RBPLJ0136+4751 &            OC 457 &  01:36:58.6 &  $+$47:51:29.0 &                       0.859 &  \cite{1987ApJS...63....1H} &      3 &    v &   64 &  4 &   3 &   8.75 &  0.64 &  0.86 &     - \\
 RBPLJ0152+0146 &          RBS 0248 &  01:52:39.6 &  $+$01:47:17.4 &                        0.08 &  \cite{1998ApJS..118..127L} &      6 &    4 &    9 &  2 &  20 &      - &     - &     - &     - \\
 RBPLJ0211+1051 &                 - &  02:11:13.2 &  $+$10:51:35.0 &      0.2\textsuperscript{*} &  \cite{2010ApJ...712...14M} &      3 &    v &   65 &  4 &   3 &  14.98 &  0.51 &  0.31 & -30.0 \\
 RBPLJ0217+0837 &                 - &  02:17:17.1 &  $+$08:37:03.9 &                       0.085 &  \cite{2013ApJ...764..135S} &      3 &    v &   62 &  4 &   3 &   6.11 &  0.47 &  0.50 &  76.0 \\
 RBPLJ0221+3556 &        S4 0218+35 &  02:21:05.5 &  $+$35:56:13.9 &                       0.944 &  \cite{2003ApJ...583...67C} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0222+4302 &            3C 66A &  02:22:39.6 &  $+$43:02:07.8 &                        0.37 &  \cite{2013ApJ...766...35F} &    5,6 &    v &   25 &  2 &   6 &   7.99 &  0.40 &  0.38 &  16.0 \\
 RBPLJ0232+2017 &                 - &  02:32:48.6 &  $+$20:17:17.4 &                        0.14 &  \cite{1993ApJ...412..541S} &      6 &    4 &    8 &  2 &  18 &      - &     - &     - &     - \\
 RBPLJ0238+1636 &       AO 0235+164 &  02:38:38.9 &  $+$16:36:59.0 &                        0.94 &  \cite{1987ApJS...63....1H} &      5 &    v &   20 &  3 &   5 &  12.15 &  0.49 &  0.39 &  22.0 \\
 RBPLJ0259+0747 &      PKS 0256+075 &  02:59:27.1 &  $+$07:47:39.6 &                       0.893 &  \cite{1993MNRAS.264..298M} &      3 &    v &   34 &  3 &   5 &  23.59 &  0.47 &  0.07 &  53.0 \\
 RBPLJ0303+4716 &       B3 0300+470 &  03:03:35.2 &  $+$47:16:16.3 &                       0.475 &  \cite{1992ApJ...396..469H} &      5 &    v &   15 &  3 &  10 &   7.25 &  0.45 &  0.40 &  81.0 \\
 RBPLJ0303-2407 &      PKS 0301-243 &  03:03:26.5 &  $-$24:07:11.5 &                      0.2657 &  \cite{2014AnA...565A..12P} &      3 &    v &   12 &  3 &  17 &   6.67 &  0.24 &  0.19 &  54.0 \\
 RBPLJ0316+4119 &      TXS 0313+411 &  03:16:43.0 &  $+$41:19:29.9 &                     0.01894 &  \cite{2002AJ....123.2990B} &      5 &    4 &    8 &  2 &  19 &      - &     - &     - &     - \\
 RBPLJ0319+1845 &          RBS 0413 &  03:19:51.8 &  $+$18:45:34.4 &                        0.19 &  \cite{1991ApJS...76..813S} &    5,6 &    v &    7 &  3 &  12 &      - &     - &     - &     - \\
 RBPLJ0319+4130 &          NGC 1275 &  03:19:48.2 &  $+$41:30:42.1 &                     0.01756 &  \cite{1992ApJS...83...29S} &      5 &    4 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0324+3410 &        J0324+3410 &  03:24:41.1 &  $+$34:10:46.0 &                       0.061 &  \cite{1996MNRAS.281..425M} &      5 &    4 &   29 &  4 &   7 &   1.09 &  0.51 &  0.24 &  -8.0 \\
 RBPLJ0336+3218 &         4C +32.14 &  03:36:30.1 &  $+$32:18:29.0 &                       1.263 &  \cite{1987ApJS...63....1H} &      5 &    v &    7 &  2 &  15 &      - &     - &     - &     - \\
 RBPLJ0339-0146 &       PKS 0336-01 &  03:39:30.9 &  $-$01:46:35.8 &                       0.852 &  \cite{1978ApJS...36..317W} &      5 &    v &    4 &  1 &   6 &      - &     - &     - &     - \\
 RBPLJ0340-2119 &      PKS 0338-214 &  03:40:35.6 &  $-$21:19:31.2 &                       0.223 &  \cite{2005AJ....129..559S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0405-1308 &       PKS 0403-13 &  04:05:34.0 &  $-$13:08:13.7 &                     0.57055 &  \cite{1996ApJS..104...37M} &      3 &    v &   22 &  3 &   6 &   1.61 &  0.46 &  0.21 & -17.0 \\
 RBPLJ0407+0742 &                 - &  04:07:29.1 &  $+$07:42:07.5 &                       1.133 &  \cite{2003ApJ...590..109S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0416+0105 &      1ES 0414+009 &  04:16:52.5 &  $+$01:05:23.9 &                       0.287 &  \cite{2011NewA...16..503M} &      6 &    v &    4 &  2 &  36 &      - &     - &     - &     - \\
 RBPLJ0423-0120 &       PKS 0420-01 &  04:23:15.8 &  $-$01:20:33.1 &                     0.91609 &  \cite{2009MNRAS.399..683J} &      3 &    v &   21 &  3 &   5 &  10.00 &  0.55 &  0.71 &     - \\
 RBPLJ0442-0017 &                 - &  04:42:38.7 &  $+$00:17:43.4 &                       0.844 &  \cite{1987ApJS...63....1H} &      5 &    v &   15 &  2 &   6 &   6.32 &  0.52 &  0.31 &  -1.0 \\
 RBPLJ0507+6737 &      1ES 0502+675 &  05:07:56.2 &  $+$67:37:24.4 &                        0.34 &  \cite{2013ApJ...764..135S} &      6 &    v &   15 &  3 &   6 &   4.12 &  0.25 &  0.14 & -64.0 \\
 RBPLJ0509+0541 &                 - &  05:09:26.0 &  $+$05:41:35.3 &                      0.3365 &  \cite{2018ApJ...854L..32P} &      5 &    v &    6 &  1 &   1 &      - &     - &     - &     - \\
 RBPLJ0510+1800 &       PKS 0507+17 &  05:10:02.4 &  $+$18:00:41.6 &                       0.416 &  \cite{1998AJ....115.1253P} &      5 &    v &    2 &  1 &  13 &      - &     - &     - &     - \\
 RBPLJ0521+2112 &      TXS 0518+211 &  05:21:52.3 &  $+$21:14:10.1 &                       0.108 &  \cite{2013ApJ...764..135S} &      6 &    v &   27 &  3 &   1 &   6.34 &  0.46 &  0.30 &  31.0 \\
 RBPLJ0642+6758 &                 - &  06:42:04.0 &  $+$67:58:35.4 &                        3.18 &  \cite{1994ApJ...436..678O} &      4 &    v &   25 &  3 &   5 &   0.90 &  0.53 &  0.30 & -13.0 \\
 RBPLJ0648+1516 &     VER J0648+152 &  06:48:47.6 &  $+$15:16:24.8 &                       0.179 &  \cite{2011ApJ...742..127A} &      6 &    v &    3 &  2 &   2 &      - &     - &     - &     - \\
 RBPLJ0650+2502 &      1ES 0647+250 &  06:50:46.5 &  $+$25:02:59.6 &                       0.203 &  \cite{2012ApJ...744..177L} &      6 &    v &    5 &  2 &  14 &      - &     - &     - &     - \\
 RBPLJ0702+8549 &                 - &  07:02:32.8 &  $+$85:49:52.5 &                       1.059 &  \cite{2008ApJS..175...97H} &      2 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0710+5908 &      TXS 0706+592 &  07:10:30.1 &  $+$59:08:20.4 &                       0.125 &  \cite{2011NewA...16..503M} &      6 &    4 &   12 &  2 &  12 &   4.12 &  0.27 &  0.16 &  17.0 \\
 RBPLJ0721+7120 &        S5 0716+71 &  07:21:53.4 &  $+$71:20:36.4 &                        0.31 &  \cite{2008AnA...487L..29N} &      5 &    v &   57 &  4 &   2 &  11.37 &  0.43 &  0.53 &     - \\
 RBPLJ0728+5701 &                 - &  07:28:49.6 &  $+$57:01:24.4 &                       0.426 &  \cite{1997MNRAS.290..380H} &      5 &    4 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0738+1742 &       PKS 0735+17 &  07:38:07.4 &  $+$17:42:19.0 &                        0.45 &  \cite{2012AnA...547A...1N} &      5 &    v &   12 &  3 &   7 &   7.70 &  0.44 &  0.12 &  25.0 \\
 RBPLJ0750+1231 &            OI 280 &  07:50:52.0 &  $+$12:31:04.8 &                       0.889 &  \cite{1987ApJS...63....1H} &      5 &    v &   12 &  3 &  13 &   4.11 &  0.47 &  0.51 &     - \\
 RBPLJ0809+5218 &      1ES 0806+524 &  08:09:49.2 &  $+$52:18:58.2 &                       0.138 &  \cite{1998AnA...334..459B} &      6 &    v &    5 &  2 &  43 &      - &     - &     - &     - \\
 RBPLJ0814+6431 &                 - &  08:14:39.2 &  $+$64:31:22.0 &                       0.239 &  \cite{2013ApJ...764..135S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0818+4222 &      TXS 0814+425 &  08:18:16.0 &  $+$42:22:45.4 &                       0.530 &  \cite{2005ApJ...626...95S} &      5 &    v &   10 &  2 &   6 &      - &     - &     - &     - \\
 RBPLJ0825+6157 &      TXS 0821+621 &  08:25:38.6 &  $+$61:57:28.6 &                       0.542 &  \cite{1987ApJS...63....1H} &      4 &    v &   14 &  3 &  14 &   2.81 &  0.28 &  0.14 & -19.0 \\
 RBPLJ0830+2410 &            OJ 248 &  08:30:52.1 &  $+$24:10:59.8 &                      0.9414 &  \cite{2010MNRAS.405.2302H} &      5 &    v &   13 &  3 &   4 &   1.58 &  0.64 &  0.30 &  -5.0 \\
 RBPLJ0837+5825 &        S4 0833+58 &  08:37:22.4 &  $+$58:25:01.8 &                       2.101 &  \cite{2008ApJS..175...97H} &      5 &    v &    2 &  1 &  10 &      - &     - &     - &     - \\
 RBPLJ0841+7053 &         4C +71.07 &  08:41:24.4 &  $+$70:53:42.2 &                       2.172 &  \cite{1993AnAS..100..395S} &    1,3 &    v &   29 &  3 &   6 &   2.55 &  0.76 &  0.25 &  -5.0 \\
 RBPLJ0848+6606 &                 - &  08:48:54.6 &  $+$66:06:09.5 &                           - &                           - &  1,3,6 &    v &   24 &  3 &   7 &   7.29 &  0.37 &  0.27 &  39.0 \\
 RBPLJ0849+5108 &        J0849+5108 &  08:49:58.0 &  $+$51:08:29.0 &                      0.5847 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    5 &  2 &   5 &      - &     - &     - &     - \\
 RBPLJ0854+2006 &            OJ 287 &  08:54:48.9 &  $+$20:06:30.6 &                      0.3056 &  \cite{2010AnA...516A..60N} &      5 &    4 &   39 &  3 &   2 &  12.35 &  0.52 &  0.49 & -17.0 \\
 RBPLJ0854+5757 &        S4 0850+58 &  08:54:42.0 &  $+$57:57:29.9 &                     1.31915 &  \cite{2010MNRAS.405.2302H} &      4 &    v &   12 &  3 &  10 &   3.44 &  0.58 &  0.20 &  -5.0 \\
 RBPLJ0948+0022 &        J0948+0022 &  09:48:57.3 &  $+$00:22:25.6 &                      0.5851 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    7 &  3 &   9 &      - &     - &     - &     - \\
 RBPLJ0956+2515 &      TXS 0953+254 &  09:56:49.9 &  $+$25:15:16.1 &                    0.707208 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ0957+5522 &         4C +55.17 &  09:57:38.2 &  $+$55:22:57.8 &                     0.89961 &  \cite{2010MNRAS.405.2302H} &    1,3 &    v &   13 &  3 &  13 &   4.57 &  0.44 &  0.14 &  13.0 \\
 RBPLJ0958+6533 &        S4 0954+65 &  09:58:47.2 &  $+$65:33:54.8 &    0.368\textsuperscript{*} &  \cite{1992ApJ...398..454W} &      3 &    v &   19 &  3 &  10 &  13.68 &  0.35 &  0.16 &   2.0 \\
 RBPLJ1010+8250 &        S5 1003+83 &  10:10:15.8 &  $+$82:50:14.4 &                       0.322 &  \cite{1994AJ....108..395X} &      2 &    v &    2 &  1 & 130 &      - &     - &     - &     - \\
 RBPLJ1012+0630 &      TXS 1009+067 &  10:12:13.3 &  $+$06:30:57.2 &                       0.727 &  \cite{2005AJ....129..559S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1014+2301 &      PKS 1012+232 &  10:14:47.1 &  $+$23:01:16.6 &                    0.566402 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    2 &  1 &   3 &      - &     - &     - &     - \\
 RBPLJ1017+6116 &      TXS 1013+615 &  10:17:25.9 &  $+$61:16:27.5 &                    2.800565 &  \cite{2010MNRAS.405.2302H} &      2 &    v &    2 &  1 & 127 &      - &     - &     - &     - \\
 RBPLJ1018+3542 &        S4 1015+35 &  10:18:11.0 &  $+$35:42:39.4 &                    1.229508 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1023+3948 &        S4 1020+40 &  10:23:11.6 &  $+$39:48:15.4 &                       1.254 &  \cite{1994AJ....108..395X} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1032+3738 &      TXS 1029+378 &  10:32:40.7 &  $+$37:38:27.0 &                       0.528 &  \cite{2010AJ....139..390P} &      1 &    v &    3 &  1 &   2 &      - &     - &     - &     - \\
 RBPLJ1033+6051 &        S4 1030+61 &  10:33:51.4 &  $+$60:51:07.3 &                    1.409276 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1037+5711 &                 - &  10:37:44.3 &  $+$57:11:55.6 &  0.83037\textsuperscript{*} &  \cite{2009AJ....137.3884R} &  1,3,6 &    v &   25 &  3 &   8 &   3.73 &  0.54 &  0.86 &     - \\
 RBPLJ1041+0610 &      PKS 1038+064 &  10:41:17.2 &  $+$06:10:16.9 &                       1.265 &  \cite{2008ApJS..175...97H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1048+7143 &        S5 1044+71 &  10:48:27.6 &  $+$71:43:35.9 &                       1.150 &  \cite{1995ApJS...98....1P} &    1,3 &    v &   43 &  3 &   1 &  13.00 &  0.66 &  0.95 &     - \\
 RBPLJ1054+2210 &                 - &  10:54:30.6 &  $+$22:10:54.9 &    2.055\textsuperscript{*} &  \cite{2009ApJS..180...67R} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1058+0133 &       PKS 1055+01 &  10:58:29.6 &  $+$01:33:58.8 &                        0.89 &  \cite{2004MNRAS.349.1397C} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1058+5628 &      TXS 1055+567 &  10:58:37.7 &  $+$56:28:11.2 &    0.143\textsuperscript{*} &  \cite{2013ApJ...764..135S} &      3 &    v &   18 &  3 &   9 &   3.85 &  0.62 &  0.67 &     - \\
 RBPLJ1059-1134 &     PKS B1056-113 &  10:59:12.4 &  $-$11:34:22.8 &     0.27\textsuperscript{l} &  \cite{2013AJ....145..114L} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1104+0730 &    PMN J1104+0730 &  11:04:24.1 &  $+$07:30:53.2 &    1.033\textsuperscript{m} &  \cite{2017ApJS..233...25A} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1104+3812 &           Mkn 421 &  11:04:27.3 &  $+$38:12:31.8 &                    0.029316 &  \cite{2015ApJS..218...10V} &      5 &    6 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1121-0553 &       PKS 1118-05 &  11:21:25.1 &  $-$05:53:56.4 &                       1.297 &  \cite{1997MNRAS.284...85D} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1132+0034 &      TXS 1130+008 &  11:32:45.6 &  $+$00:34:27.8 &                       1.223 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    2 &  1 &  15 &      - &     - &     - &     - \\
 RBPLJ1136+7009 &        S5 1133+70 &  11:36:26.4 &  $+$70:09:27.3 &                     0.04528 &  \cite{1999PASP..111..438F} &      6 &    4 &   18 &  2 &   5 &   2.69 &  0.45 &  0.52 &     - \\
 RBPLJ1148+5924 &          NGC 3894 &  11:48:50.4 &  $+$59:24:56.4 &                     0.01075 &  \cite{1979ApJS...40..527P} &      2 &    6 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1152-0841 &      TXS 1149-084 &  11:52:17.2 &  $-$08:41:03.3 &                       2.367 &  \cite{2008ApJS..175...97H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1159+2914 &      TXS 1156+295 &  11:59:31.8 &  $+$29:14:43.8 &                      0.7247 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    2 &  2 &   - &      - &     - &     - &     - \\
 RBPLJ1203+6031 &                 - &  12:03:03.5 &  $+$60:31:19.2 &                      0.0656 &  \cite{1998ApJ...494...47F} &  1,3,6 &    4 &   26 &  3 &   9 &   1.46 &  0.49 &  0.26 &  34.0 \\
 RBPLJ1204-0710 &                 - &  12:04:16.7 &  $-$07:10:09.0 &                      0.1838 &  \cite{2001PASA...18..232M} &      1 &    4 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1217+3007 &        B2 1215+30 &  12:17:52.1 &  $+$30:07:01.0 &                       0.130 &  \cite{2003ApJS..148..275A} &    1,6 &    5 &   16 &  2 &   6 &  10.04 &  0.18 &  0.04 & -20.0 \\
 RBPLJ1220+0203 &       PKS 1217+02 &  12:20:11.9 &  $+$02:03:42.2 &                      0.2404 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1221+2813 &             W Com &  12:21:31.7 &  $+$28:13:58.5 &                       0.103 &  \cite{2013ApJ...764..135S} &      6 &    5 &    9 &  3 &  11 &      - &     - &     - &     - \\
 RBPLJ1221+3010 &        H 1219+305 &  12:21:21.9 &  $+$30:10:37.1 &                       0.182 &  \cite{1998AnA...334..459B} &      6 &    5 &    7 &  2 &  15 &      - &     - &     - &     - \\
 RBPLJ1222+0413 &       PKS 1219+04 &  12:22:22.5 &  $+$04:13:15.8 &                       0.965 &  \cite{2008ApJS..175...97H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1224+2122 &       PKS 1222+21 &  12:24:54.5 &  $+$21:22:46.4 &                       0.432 &  \cite{1987ApJ...323..108O} &      5 &    v &    8 &  2 &  16 &      - &     - &     - &     - \\
 RBPLJ1224+2436 &     RGB J1224+246 &  12:24:24.2 &  $+$24:36:23.6 &                       0.218 &  \cite{1991ApJS...76..813S} &    1,6 &    v &    7 &  3 &  18 &      - &     - &     - &     - \\
 RBPLJ1229+0203 &            3C 273 &  12:29:06.7 &  $+$02:03:08.6 &                     0.15834 &  \cite{1992ApJS...83...29S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1230+2518 &        S3 1227+25 &  12:30:14.1 &  $+$25:18:07.1 &                       0.135 &  \cite{1996AnA...309..419N} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1231+2847 &      TXS 1229+290 &  12:31:43.6 &  $+$28:47:49.8 &                       0.236 &  \cite{2003AnA...401..927B} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1238-1959 &    PMN J1238-1959 &  12:38:24.4 &  $-$19:59:13.6 &                           - &                           - &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1245+5709 &                 - &  12:45:10.0 &  $+$57:09:54.4 &                     1.54487 &  \cite{2009ApJS..182..543A} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1248+5820 &      TXS 1246+586 &  12:48:18.8 &  $+$58:20:28.7 &                      0.8474 &              \cite{SDSSDR3} &    1,3 &    v &   27 &  3 &   5 &   4.85 &  0.41 &  0.36 & -55.0 \\
 RBPLJ1253+5301 &                 - &  12:53:11.9 &  $+$53:01:11.7 &                       0.445 &  \cite{2009ApJS..180...67R} &      1 &    v &    2 &  1 &   2 &      - &     - &     - &     - \\
 RBPLJ1256-0547 &            3C 279 &  12:56:11.2 &  $-$05:47:21.5 &                      0.5362 &  \cite{1996ApJS..104...37M} &    1,5 &    v &   20 &  2 &   4 &  18.71 &  0.21 &  0.08 &  48.0 \\
 RBPLJ1305+5116 &                 - &  13:05:22.7 &  $+$51:16:40.3 &                     0.78755 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    2 &  1 &  31 &      - &     - &     - &     - \\
 RBPLJ1337-1257 &      PKS 1335-127 &  13:37:39.8 &  $-$12:57:24.7 &                       0.539 &  \cite{1993AnAS...97..483S} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1353+7532 &                 - &  13:53:23.2 &  $+$75:32:57.7 &                       1.619 &  \cite{2008ApJS..175...97H} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1354-1041 &      PKS 1352-104 &  13:54:46.5 &  $-$10:41:02.7 &                       0.332 &  \cite{1975MNRAS.173p..87B} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1357+0128 &                 - &  13:57:38.7 &  $+$01:28:13.6 &                      0.2187 &  \cite{2005ApJ...626...95S} &      1 &    v &    2 &  1 &   2 &      - &     - &     - &     - \\
 RBPLJ1419+5423 &       PG 1418+546 &  14:19:46.6 &  $+$54:23:14.8 &                     0.15256 &              \cite{SDSSDR3} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1427+2348 &        B2 1424+24 &  14:27:00.4 &  $+$23:48:00.0 &                      0.6035 &  \cite{2015MNRAS.449.1018Y} &    1,6 &    v &   12 &  3 &  20 &   5.54 &  0.60 &  0.66 &     - \\
 RBPLJ1428+4240 &      1ES 1426+428 &  14:28:32.7 &  $+$42:40:20.6 &                      0.1291 &              \cite{SDSSDR3} &      6 &    4 &   13 &  2 &  14 &   1.85 &  0.38 &  0.27 & -23.0 \\
 RBPLJ1436+6336 &                 - &           - &            $-$ &                           - &                           - &      - &    - &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1442+1200 &      1ES 1440+122 &  14:42:48.3 &  $+$12:00:40.3 &                      0.1631 &              \cite{SDSSDR5} &      6 &  4.5 &   11 &  2 &  19 &   1.92 &  0.35 &  0.26 & -42.0 \\
 RBPLJ1505+0326 &    PMN J1505+0326 &  15:05:06.5 &  $+$03:26:30.8 &                      0.4079 &  \cite{2010MNRAS.405.2302H} &      5 &    4 &   23 &  4 &  13 &   5.04 &  0.61 &  0.45 &  -9.0 \\
 RBPLJ1510-0543 &       PKS 1508-05 &  15:10:53.6 &  $-$05:43:07.4 &                       1.185 &  \cite{1986MNRAS.218..331W} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1512+0203 &      PKS 1509+022 &  15:12:15.7 &  $+$02:03:17.0 &                     0.21991 &  \cite{2010MNRAS.405.2302H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1512-0905 &      PKS 1510-089 &  15:12:50.5 &  $-$09:05:59.8 &                       0.360 &  \cite{1990PASP..102.1235T} &    1,3 &    v &   98 &  5 &   2 &   5.13 &  0.66 &  0.96 &     - \\
 RBPLJ1516+1932 &      PKS 1514+197 &  15:16:56.8 &  $+$19:32:13.0 &                        1.07 &  \cite{2000AnARv..10...81V} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1517-2422 &            AP Lib &  15:17:41.8 &  $-$24:22:19.5 &                       0.048 &  \cite{2008ApJS..175...97H} &      5 &    6 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1526+6650 &                 - &  15:26:42.9 &  $+$66:50:54.6 &                        3.02 &  \cite{1996MNRAS.282.1274H} &      2 &    v &    2 &  1 &  50 &      - &     - &     - &     - \\
 RBPLJ1542+6129 &                 - &  15:42:56.9 &  $+$61:29:55.4 &    0.117\textsuperscript{*} &  \cite{2011ApJ...740...98M} &  1,3,6 &    v &   67 &  4 &   4 &  10.08 &  0.63 &  0.31 & -39.0 \\
 RBPLJ1548+3511 &      TXS 1546+353 &  15:48:17.9 &  $+$35:11:28.1 &                       0.479 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1548-2251 &    PMN J1548-2251 &  15:48:49.8 &  $-$22:51:02.5 &                       0.192 &  \cite{2013ApJ...764..135S} &      1 &    5 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1550+0527 &      TXS 1548+056 &  15:50:35.3 &  $+$05:27:10.4 &                       1.422 &  \cite{2008ApJS..175...97H} &      1 &    v &    2 &  1 &  16 &      - &     - &     - &     - \\
 RBPLJ1551+5806 &                 - &  15:51:58.2 &  $+$58:06:44.5 &                       1.324 &  \cite{1999MNRAS.307..149S} &    2,4 &    v &   43 &  3 &   6 &   1.28 &  0.43 &  0.27 & -34.0 \\
 RBPLJ1553+1256 &      PKS 1551+130 &  15:53:32.7 &  $+$12:56:51.7 &    1.308\textsuperscript{*} &  \cite{2014MNRAS.438.3058R} &      3 &    v &   47 &  3 &   7 &   1.83 &  0.64 &  0.25 & -16.0 \\
 RBPLJ1555+1111 &       PG 1553+113 &  15:55:43.0 &  $+$11:11:24.4 &    0.360\textsuperscript{*} &  \cite{2011ApJS..194...29R} &  1,3,6 &    v &  284 &  5 &   0 &   3.29 &  0.43 &  0.28 &   0.0 \\
 RBPLJ1558+5625 &      TXS 1557+565 &  15:58:48.3 &  $+$56:25:14.1 &    0.300\textsuperscript{*} &  \cite{1998ApJ...494...47F} &  1,3,6 &    v &   48 &  3 &   7 &   6.63 &  0.44 &  0.95 &     - \\
 RBPLJ1603+5730 &         4C +57.27 &  16:03:55.9 &  $+$57:30:54.4 &   2.4084\textsuperscript{*} &  \cite{1991ApJS...77..203J} &    2,4 &    v &   31 &  3 &   9 &   1.04 &  0.55 &  0.50 & -14.0 \\
 RBPLJ1604+5714 &                 - &  16:04:37.4 &  $+$57:14:36.7 &                       0.720 &  \cite{1998ApJ...494...47F} &    1,3 &    v &   37 &  3 &   9 &   3.37 &  0.71 &  0.34 & -17.0 \\
 RBPLJ1607+1551 &         4C +15.54 &  16:07:06.4 &  $+$15:51:34.5 &   0.4965\textsuperscript{*} &              \cite{SDSSDR6} &      3 &    v &   39 &  3 &   9 &   7.09 &  0.45 &  0.78 &     - \\
 RBPLJ1608+1029 &      TXS 1606+105 &  16:08:46.2 &  $+$10:29:07.8 &                       1.226 &  \cite{2008ApJS..175...97H} &      1 &    v &    3 &  1 &  13 &      - &     - &     - &     - \\
 RBPLJ1623+6624 &                 - &  16:23:04.5 &  $+$66:24:01.1 &                       0.203 &  \cite{2007AnA...463...97L} &      2 &    v &    2 &  1 & 124 &      - &     - &     - &     - \\
 RBPLJ1624+5652 &                 - &  16:24:32.2 &  $+$56:52:28.0 &    0.415\textsuperscript{*} &  \cite{2009ApJS..180...67R} &    2,4 &    v &   35 &  3 &   7 &   9.69 &  0.38 &  0.26 &  32.0 \\
 RBPLJ1628+4007 &   EXO 1627.3+4014 &  16:29:01.3 &  $+$40:07:59.9 &                      0.2725 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    2 &  1 &  45 &      - &     - &     - &     - \\
 RBPLJ1633+4718 &                 - &  16:33:23.6 &  $+$47:18:58.9 &                      0.1158 &  \cite{2017ApJS..229...39R} &      5 &    4 &    4 &  1 &  14 &      - &     - &     - &     - \\
 RBPLJ1635+3808 &         4C +38.41 &  16:35:15.5 &  $+$38:08:04.5 &                      1.8131 &  \cite{2010MNRAS.405.2302H} &    1,3 &    v &   99 &  4 &   2 &   7.26 &  0.63 &  0.81 &     - \\
 RBPLJ1637+4717 &        S4 1636+47 &  16:37:45.1 &  $+$47:17:33.8 &                      0.7354 &  \cite{2015MNRAS.452.4153A} &      1 &    v &    3 &  1 &   3 &      - &     - &     - &     - \\
 RBPLJ1638+5720 &        S4 1637+57 &  16:38:13.5 &  $+$57:20:24.0 &                      0.7506 &  \cite{1996ApJS..104...37M} &    2,4 &    v &   40 &  3 &   9 &   0.74 &  0.68 &  0.47 &   0.0 \\
 RBPLJ1640+3946 &        S4 1638+39 &  16:40:29.6 &  $+$39:46:46.0 &                       1.666 &  \cite{2008ApJS..175...97H} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1642+3948 &            3C 345 &  16:42:58.8 &  $+$39:48:37.0 &                      0.5928 &  \cite{1996ApJS..104...37M} &    1,3 &    v &   44 &  4 &   8 &   5.54 &  0.48 &  0.31 &  53.0 \\
 RBPLJ1643-0646 &                 - &  16:43:28.9 &  $-$06:46:19.4 &                           - &                           - &      1 &    6 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1644+2619 &     RGB J1644+263 &  16:44:42.5 &  $+$26:19:13.3 &                       0.145 &  \cite{1995AnAS..110..469B} &      5 &    v &    4 &  1 &  14 &      - &     - &     - &     - \\
 RBPLJ1649+5235 &                 - &  16:49:25.0 &  $+$52:35:15.0 &                       2.055 &  \cite{2009ApJS..180...67R} &    1,6 &    v &   49 &  3 &   7 &   5.71 &  0.47 &  0.67 &     - \\
 RBPLJ1653+3945 &           MRK 501 &  16:53:52.2 &  $+$39:45:36.6 &                     0.03366 &  \cite{1993AnAS...98..393S} &    1,3 &    6 &   73 &  3 &   4 &   2.29 &  0.38 &  0.25 & -41.0 \\
 RBPLJ1722+1013 &      TXS 1720+102 &  17:22:44.6 &  $+$10:13:35.8 &                       0.732 &  \cite{2003ARep...47..903G} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1722+5654 &                 - &  17:22:06.0 &  $+$56:54:51.6 &                       0.426 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    3 &  1 &  18 &      - &     - &     - &     - \\
 RBPLJ1725+1152 &        H 1722+119 &  17:25:04.3 &  $+$11:52:15.5 &    0.018\textsuperscript{*} &  \cite{1993ApJS...85..111C} &    3,6 &    v &   89 &  4 &   3 &   7.19 &  0.56 &  0.38 &  42.0 \\
 RBPLJ1727+4530 &        S4 1726+45 &  17:27:27.7 &  $+$45:30:39.7 &                       0.717 &  \cite{1997MNRAS.290..380H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1727+5510 &                 - &  17:27:23.5 &  $+$55:10:53.5 &                       0.247 &  \cite{2008ApJS..175...97H} &      5 &    4 &    4 &  1 &  17 &      - &     - &     - &     - \\
 RBPLJ1728+0427 &      TXS 1725+044 &  17:28:25.0 &  $+$04:27:04.9 &                       0.293 &  \cite{2008ApJS..175...97H} &      5 &    4 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1728+5013 &           OT +546 &  17:28:18.6 &  $+$50:13:10.5 &                      0.0554 &  \cite{1978ApJ...219L..97O} &      6 &    6 &   13 &  2 &  21 &   2.27 &  0.40 &  0.68 &     - \\
 RBPLJ1733-1304 &      PKS 1730-130 &  17:33:02.7 &  $-$13:04:49.5 &                       0.902 &  \cite{2008ApJS..175...97H} &      5 &    5 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1743+1935 &      1ES 1741+196 &  17:43:57.8 &  $+$19:35:09.0 &                       0.084 &  \cite{1999AnA...348..113H} &      6 &    5 &   12 &  2 &  23 &   2.60 &  0.43 &  0.12 &  61.0 \\
 RBPLJ1745-0753 &      TXS 1742-078 &  17:45:27.1 &  $-$07:53:03.9 &                           - &                           - &      5 &    v &    2 &  1 &  17 &      - &     - &     - &     - \\
 RBPLJ1748+7005 &        S5 1749+70 &  17:48:32.8 &  $+$70:05:50.8 &                       0.770 &  \cite{1992ApJ...396..469H} &    1,3 &    v &   94 &  4 &   3 &  10.31 &  0.43 &  0.42 & -48.0 \\
 RBPLJ1749+4321 &      TXS 1747+433 &  17:49:00.4 &  $+$43:21:51.3 &    0.215\textsuperscript{*} &  \cite{2011ApJ...740...98M} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1751+0939 &            OT 081 &  17:51:32.8 &  $+$09:39:00.7 &                       0.320 &  \cite{1993AnAS...98..393S} &      3 &    v &   96 &  4 &   3 &  10.28 &  0.58 &  0.74 &     - \\
 RBPLJ1754+3212 &                 - &  17:54:11.8 &  $+$32:12:23.1 &     1.09\textsuperscript{*} &  \cite{2013AJ....146..127S} &  1,3,6 &    v &   77 &  4 &   4 &   4.34 &  0.55 &  0.57 &     - \\
 RBPLJ1800+3848 &        S4 1758+38 &  18:00:24.8 &  $+$38:48:30.7 &                       2.092 &  \cite{1994AnAS..103..349S} &      4 &    v &   33 &  3 &  11 &   2.03 &  0.61 &  0.44 & -41.0 \\
 RBPLJ1800+7828 &        S5 1803+78 &  18:00:45.7 &  $+$78:28:04.0 &                       0.684 &  \cite{2001AJ....122..565R} &    1,3 &    v &   79 &  4 &   3 &   8.07 &  0.43 &  0.75 &     - \\
 RBPLJ1806+6949 &        S4 1807+69 &  18:06:50.7 &  $+$69:49:28.1 &                       0.051 &  \cite{1992AnAS...96..389d} &    1,3 &    6 &   84 &  4 &   3 &   5.40 &  0.46 &  0.14 &  65.0 \\
 RBPLJ1809+2041 &                 - &  18:09:25.5 &  $+$20:41:31.0 &                           - &                           - &  1,3,6 &    v &   47 &  3 &   6 &   3.26 &  0.70 &  0.79 &     - \\
 RBPLJ1813+0615 &      TXS 1811+062 &  18:13:33.4 &  $+$06:15:42.0 &     0.70\textsuperscript{*} &  \cite{2010ApJ...712...14M} &      1 &    v &    2 &  1 &  13 &      - &     - &     - &     - \\
 RBPLJ1813+3144 &      TXS 1811+317 &  18:13:35.2 &  $+$31:44:17.6 &                       0.117 &  \cite{1991ApJ...378...77G} &  1,3,6 &    v &   71 &  4 &   3 &   4.34 &  0.50 &  0.92 &     - \\
 RBPLJ1823+7938 &        S5 1826+79 &  18:23:14.1 &  $+$79:38:49.0 &                       0.224 &  \cite{1997MNRAS.290..380H} &      5 &    v &    4 &  1 &  50 &      - &     - &     - &     - \\
 RBPLJ1824+5651 &        S4 1823+56 &  18:24:07.1 &  $+$56:51:01.5 &                       0.664 &  \cite{1986AJ.....91..494L} &      1 &    v &    2 &  1 &   9 &      - &     - &     - &     - \\
 RBPLJ1835+3241 &            3C 382 &  18:35:03.4 &  $+$32:41:46.8 &                     0.05787 &  \cite{1996AJ....112.1803M} &      4 &    6 &   62 &  4 &   3 &   0.75 &  0.49 &  0.28 &  37.0 \\
 RBPLJ1836+3136 &                 - &  18:36:21.2 &  $+$31:36:26.8 &                           - &                           - &  1,3,6 &    v &   40 &  3 &   8 &   7.51 &  0.65 &  0.26 & -14.0 \\
 RBPLJ1838+4802 &                 - &  18:38:49.2 &  $+$48:02:34.3 &      0.3\textsuperscript{*} &  \cite{2003AnA...400...95N} &  1,3,6 &    v &   45 &  3 &   8 &   5.87 &  0.59 &  0.32 &  39.0 \\
 RBPLJ1841+3218 &                 - &  18:41:47.0 &  $+$32:18:39.1 &                           - &                           - &    3,6 &    v &   41 &  3 &   9 &   5.29 &  0.46 &  0.31 &  22.0 \\
 RBPLJ1844+5709 &      TXS 1843+571 &  18:44:51.2 &  $+$57:09:40.6 &                           - &                           - &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1848+3244 &      TXS 1846+326 &  18:48:34.4 &  $+$32:44:00.1 &                       0.918 &  \cite{2015ApJS..217....2M} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1849+6705 &        S4 1849+67 &  18:49:16.1 &  $+$67:05:41.7 &                       0.657 &  \cite{1993AnAS..100..395S} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1850+2825 &      TXS 1848+283 &  18:50:27.6 &  $+$28:25:13.2 &                        2.56 &  \cite{1993ApJ...407..456W} &      5 &    v &    3 &  1 &  26 &      - &     - &     - &     - \\
 RBPLJ1854+7351 &        S5 1856+73 &  18:54:57.3 &  $+$73:51:19.9 &                       0.461 &  \cite{1997MNRAS.290..380H} &    2,4 &    v &   31 &  3 &  10 &   1.46 &  0.65 &  0.17 & -17.0 \\
 RBPLJ1903+5540 &      TXS 1902+556 &  19:03:11.6 &  $+$55:40:38.5 &     0.58\textsuperscript{*} &  \cite{2010ApJ...712...14M} &  1,3,6 &    v &   76 &  4 &   3 &   9.33 &  0.48 &  0.37 &  18.0 \\
 RBPLJ1911-1908 &      TXS 1908-192 &  19:11:29.7 &  $-$19:08:23.5 &                           - &                           - &      5 &    5 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1918+4937 &                 - &  19:18:45.6 &  $+$49:37:56.0 &                       0.926 &  \cite{2008ApJS..175...97H} &      5 &    v &    3 &  1 &  43 &      - &     - &     - &     - \\
 RBPLJ1923-2104 &      TXS 1920-211 &  19:23:32.2 &  $-$21:04:33.3 &                       0.874 &  \cite{2003AJ....125..572H} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ1927+6117 &        S4 1926+61 &  19:27:30.4 &  $+$61:17:32.9 &     0.54\textsuperscript{*} &  \cite{2010ApJ...712...14M} &    1,3 &    v &   37 &  3 &   8 &   8.28 &  0.44 &  0.62 &     - \\
 RBPLJ1927+7358 &        S5 1928+73 &  19:27:48.5 &  $+$73:58:01.6 &                      0.3021 &  \cite{1996ApJS..104...37M} &    2,4 &    v &   28 &  3 &  11 &   1.72 &  0.24 &  0.07 & -32.0 \\
 RBPLJ1941-0211 &    PMN J1941-0212 &  19:41:18.9 &  $-$02:11:45.4 &                       0.202 &  \cite{2008ApJS..175...97H} &      5 &    5 &    8 &  2 &  19 &      - &     - &     - &     - \\
 RBPLJ1955+5131 &        S4 1954+51 &  19:55:42.7 &  $+$51:31:49.0 &                        1.23 &  \cite{1994AnAS..103..349S} &      4 &    v &   17 &  2 &  10 &   2.78 &  0.53 &  0.05 & -30.0 \\
 RBPLJ1959+6508 &      TXS 1959+650 &  19:59:59.9 &  $+$65:08:54.7 &                       0.047 &  \cite{1993ApJ...412..541S} &  1,3,6 &    6 &   92 &  4 &   4 &   4.21 &  0.40 &  0.29 & -36.0 \\
 RBPLJ2000-1748 &      PKS 1958-179 &  20:00:57.1 &  $-$17:48:57.7 &                        0.65 &  \cite{1975MNRAS.173p..87B} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2001+4352 &        J2001+4352 &  20:01:12.9 &  $+$43:52:52.8 &                        0.18 &  \cite{2014AnA...572A.121A} &      6 &    4 &   19 &  2 &   7 &  14.89 &  0.22 &  0.11 & -80.0 \\
 RBPLJ2005+7752 &        S5 2007+77 &  20:05:30.9 &  $+$77:52:43.1 &                       0.342 &  \cite{1989AnAS...80..103S} &    1,3 &    v &   76 &  4 &   3 &   6.00 &  0.58 &  0.52 &     - \\
 RBPLJ2015-0137 &      PKS 2012-017 &  20:15:15.2 &  $-$01:37:32.6 &                           - &                           - &  1,3,6 &    v &   40 &  3 &   8 &  14.68 &  0.31 &  0.13 &  64.0 \\
 RBPLJ2016+1632 &      TXS 2013+163 &  20:16:13.9 &  $+$16:32:34.1 &                           - &                           - &      4 &    v &   27 &  3 &  13 &   1.51 &  0.61 &  0.22 & -20.0 \\
 RBPLJ2016-0903 &                 - &  20:16:24.0 &  $-$09:03:33.0 &                       0.367 &  \cite{2011ApJ...743..171A} &    1,3 &    v &   35 &  3 &  10 &   2.46 &  0.80 &  0.18 &   2.0 \\
 RBPLJ2022+6136 &        S4 2021+61 &  20:22:06.7 &  $+$61:36:58.8 &                       0.227 &  \cite{1991ApJS...75..297H} &      5 &    4 &    7 &  1 &  15 &      - &     - &     - &     - \\
 RBPLJ2022+7611 &        S5 2023+76 &  20:22:35.6 &  $+$76:11:26.2 &                       0.594 &  \cite{2011ApJ...743..171A} &  1,3,6 &    v &   72 &  4 &   3 &  11.93 &  0.39 &  0.33 &  51.0 \\
 RBPLJ2024+1718 &                 - &  20:24:56.6 &  $+$17:18:13.2 &                        1.05 &  \cite{1996ESOSR..17....1V} &      4 &    v &   24 &  3 &  14 &   1.44 &  0.91 &  0.43 & -26.0 \\
 RBPLJ2030+1936 &     RGB J2030+196 &  20:30:57.1 &  $+$19:36:12.9 &                       0.668 &  \cite{2015ApJS..217....2M} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2030-0622 &      TXS 2027-065 &  20:30:14.8 &  $-$06:22:04.4 &                       0.667 &  \cite{2015ApJ...810...14A} &    1,3 &    v &   69 &  4 &   3 &   0.69 &  0.70 &  0.31 & -28.0 \\
 RBPLJ2031+1219 &      TXS 2029+121 &  20:31:55.0 &  $+$12:19:41.3 &                       1.215 &  \cite{1993AnAS..100..395S} &      5 &    3 &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2033+2146 &         4C +21.55 &  20:33:32.0 &  $+$21:46:22.4 &                      0.1735 &  \cite{2007ApJ...664...64I} &      4 &    4 &   18 &  2 &   7 &   5.58 &  0.15 &  0.04 & -27.0 \\
 RBPLJ2035+1056 &      TXS 2032+107 &  20:35:22.3 &  $+$10:56:06.8 &                       0.601 &  \cite{1987AJ.....93..785A} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2039-1046 &      TXS 2036-109 &  20:39:00.7 &  $-$10:46:41.7 &     1.05\textsuperscript{*} &  \cite{2013AJ....146..127S} &    1,3 &    v &   43 &  3 &   7 &   7.95 &  0.47 &  0.78 &     - \\
 RBPLJ2042+7508 &         4C +74.26 &  20:42:36.9 &  $+$75:08:01.6 &                       0.104 &  \cite{1996AnAS..115....1S} &    2,4 &    v &   42 &  3 &   8 &   1.57 &  0.21 &  0.07 &   4.0 \\
 RBPLJ2051+1742 &      PKS 2049+175 &  20:51:35.6 &  $+$17:43:36.9 &                       0.195 &  \cite{2008ApJS..175...97H} &      5 &    4 &    3 &  1 &  40 &      - &     - &     - &     - \\
 RBPLJ2131-0915 &                 - &  21:31:35.4 &  $-$09:15:23.5 &                       0.449 &  \cite{2005AnA...434..385G} &  1,3,6 &    v &   40 &  3 &   8 &   7.88 &  0.32 &  0.07 &  61.0 \\
 RBPLJ2143+1743 &        S3 2141+17 &  21:43:35.5 &  $+$17:43:48.8 &                     0.21074 &  \cite{2009ApJS..184..398H} &    1,3 &    v &   76 &  4 &   3 &   1.14 &  0.62 &  0.19 &  -1.0 \\
 RBPLJ2146-1525 &      TXS 2143-156 &  21:46:23.0 &  $-$15:25:43.9 &                       0.698 &  \cite{1997MNRAS.284...85D} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2147+0929 &        S3 2144+09 &  21:47:10.2 &  $+$09:29:46.7 &                       1.113 &  \cite{2008ApJS..175...97H} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2148+0657 &         4C +06.69 &  21:48:05.5 &  $+$06:57:38.6 &                       0.999 &  \cite{1991ApJ...382..433S} &    1,3 &    v &   70 &  4 &   3 &   1.28 &  0.72 &  0.26 & -11.0 \\
 RBPLJ2149+0322 &    PKS J2149+0323 &  21:49:41.9 &  $+$03:22:51.4 &                           - &                           - &  1,3,6 &    v &   33 &  3 &  12 &   9.86 &  0.52 &  0.96 &     - \\
 RBPLJ2150-1410 &      TXS 2147-144 &  21:50:15.5 &  $-$14:10:50.0 &                       0.229 &  \cite{1998AN....319..347F} &      3 &    5 &   29 &  3 &  11 &   2.82 &  0.48 &  0.35 & -51.0 \\
 RBPLJ2152+1734 &       PKS 2149+17 &  21:52:24.8 &  $+$17:34:37.8 &                       0.874 &  \cite{2013ApJ...764..135S} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2202+4216 &       BL Lacertae &  22:02:43.3 &  $+$42:16:40.0 &                      0.0686 &  \cite{1995ApJ...452L...5V} &    1,3 &    6 &  142 &  5 &   2 &   6.61 &  0.52 &  0.37 &   7.0 \\
 RBPLJ2217+2421 &      TXS 2214+241 &  22:17:00.8 &  $+$24:21:46.0 &                       0.505 &  \cite{2005ApJ...626...95S} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2225-0457 &            3C 446 &  22:25:47.3 &  $-$04:57:01.4 &                       1.404 &  \cite{1983MNRAS.205..793W} &      3 &    v &   33 &  3 &  10 &   5.95 &  0.86 &  0.23 & -14.0 \\
 RBPLJ2229-0832 &      TXS 2227-088 &  22:29:40.1 &  $-$08:32:54.4 &                      1.5605 &  \cite{2010MNRAS.405.2302H} &      5 &    v &    7 &  1 &  20 &      - &     - &     - &     - \\
 RBPLJ2232+1143 &           CTA 102 &  22:32:36.4 &  $+$11:43:50.9 &                       1.037 &  \cite{1965ApJ...141.1295S} &    1,3 &    v &  110 &  5 &   3 &   5.06 &  0.65 &  0.61 &     - \\
 RBPLJ2243+2021 &                 - &  22:43:54.7 &  $+$20:21:03.8 &     0.39\textsuperscript{*} &  \cite{2010ApJ...712...14M} &      3 &    v &   78 &  4 &   3 &   4.85 &  0.57 &  0.34 &  40.0 \\
 RBPLJ2250+3825 &       B3 2247+381 &  22:50:05.8 &  $+$38:24:37.2 &                      0.1187 &  \cite{1998ApJ...494...47F} &      6 &    5 &    8 &  2 &  19 &      - &     - &     - &     - \\
 RBPLJ2251+4030 &                 - &  22:51:59.8 &  $+$40:30:58.2 &                       0.229 &  \cite{2011ApJ...743..171A} &      3 &    v &   50 &  3 &   7 &   6.24 &  0.45 &  0.21 & -37.0 \\
 RBPLJ2253+1404 &                 - &  22:53:54.2 &  $+$14:04:36.9 &                       0.327 &  \cite{2010AJ....139..390P} &      5 &    v &    2 &  1 &   4 &      - &     - &     - &     - \\
 RBPLJ2253+1608 &          3C 454.3 &  22:53:57.7 &  $+$16:08:53.6 &                       0.859 &  \cite{1991MNRAS.250..414J} &    1,3 &    v &  164 &  5 &   1 &   5.90 &  0.55 &  0.56 &     - \\
 RBPLJ2311+3425 &        B2 2308+34 &  23:11:05.3 &  $+$34:25:10.9 &                       1.817 &  \cite{1976ApJS...31..143W} &      3 &    v &   48 &  3 &   1 &  16.69 &  0.78 &  0.40 & -18.0 \\
 RBPLJ2321+2732 &      TXS 2319+272 &  23:21:59.9 &  $+$27:32:46.4 &                       1.253 &  \cite{1992AnA...264...68S} &      1 &    v &    2 &  1 &   2 &      - &     - &     - &     - \\
 RBPLJ2325+3957 &       B3 2322+396 &  23:25:17.9 &  $+$39:57:36.5 &     1.04\textsuperscript{m} &  \cite{2009ApJ...704..477S} &      1 &    v &    1 &  1 &   - &      - &     - &     - &     - \\
 RBPLJ2334+0736 &      TXS 2331+073 &  23:34:12.8 &  $+$07:36:27.6 &                       0.401 &  \cite{2005ApJ...626...95S} &      3 &    v &   32 &  3 &  10 &   1.85 &  0.85 &  0.53 &     - \\
 RBPLJ2340+8015 &                 - &  23:40:54.3 &  $+$80:15:16.0 &                       0.274 &  \cite{2002ApJ...566..181C} &  1,3,6 &    v &   46 &  3 &   7 &   6.22 &  0.54 &  0.35 & -30.0 \\
 RBPLJ2347+5142 &      TXS 2344+514 &  23:47:04.8 &  $+$51:42:17.9 &                       0.044 &  \cite{1995MNRAS.277.1477P} &      6 &    5 &   11 &  2 &  16 &   2.29 &  0.44 &  0.35 & -26.0 \\
 RBPLJ2348-1631 &      TXS 2345-167 &  23:48:02.6 &  $-$16:31:12.0 &                       0.576 &  \cite{1993MNRAS.263..999T} &      5 &    v &    1 &  1 &   - &      - &     - &     - &     - \\

